Heuristics for Planning, Plan Recognition and Parsing

In a recent paper, we have shown that Plan Recognition over STRIPS can be formulated and solved using Classical Planning heuristics and algorithms. In this work, we show that this formulation subsumes the standard formulation of Plan Recognition over libraries through a compilation of libraries into STRIPS theories. The libraries correspond to AND/OR graphs that may be cyclic and where children of AND nodes may be partially ordered. These libraries include Context-Free Grammars as a special case, where the Plan Recognition problem becomes a parsing with missing tokens problem. Plan Recognition over the standard libraries become Planning problems that can be easily solved by any modern planner, while recognition over more complex libraries, including Context-Free Grammars (CFGs), illustrate limitations of current Planning heuristics and suggest improvements that may be relevant in other Planning problems too.

==> encoding.tex <==
\appendix

\section{Appendix}

{\small

Calls from \textsc{And} nodes $n$ to non--terminal children $n'$ are represented by $start(n,n',i)$ actions with precondition 
\begin{equation}
\begin{split}
Pre &= \{ top(i), started(n,i), \neg finished(n') \} \\
  & \cup \{ finished(n'', i) | n'' < n'\} \\
 & \cup \{ \neg started(n'', i) | n'' \in children(n) \}
\end{split}
\end{equation}
add list $Add = \{ top(i+1), started(n',i+1\}$ and delete list $Del = \{top(i)\}$. For calls to terminal children $n'$, the precondition of $start(n,n',i)$ is the same as the one described above but $Add = \{ finished(n',i) \}$ and $Del = \emptyset$. Termination of calls made from \textsc{And} nodes $n$ are encoded with actions $end(n,i)$, with precondition:
\begin{equation}
\begin{split}
Pre &= \{ top(i), started(n,i) \} \\
    & \cup \{ finished(n') | n' \in children(n) \}
\end{split}
\end{equation}
and add list $Add = \{ finished(n,i-1), top(i-1) \}$ and delete list $Del = Pre$.

Calls from internal \textsc{Or} nodes $n$ to children $n'$ are represented by actions $start(n,n',i)$ with precondition
\begin{equation}
\begin{split}
Pre &= \{ top(i), started(n,i) \} \\
    &\cup \{ \neg finished(n'', i+1) | n'' \in children(n) \} \\
    &\cup \{ \neg started(n'', i+1) | n'' \in children(n) \} 
\end{split}
\end{equation}
add list $Add = \{ top(i+1), started(n', i+1) \}$ and delete list $Del = \{ top(i) \}$. Termination of calls from internal \textsc{Or} nodes are represented by actions $end(n,i)$ with precondition $Pre = \{ top(i), started(n,i), finished(n',i) \}$, add list $Add = \{ finished(n, i-1), top(i-1) \}$ and delete list $Del = Pre$.

Root \textsc{Or} nodes are handled in a similar way by defining action $start(n,n',i=0)$ and action $end(n,i=0)$ with the difference that the latter, rather than adding $finished(n,i-1)$, adds $finished(n,0)$.
